Regularizing a Model-based Policy Stationary Distribution to Stabilize Offline Reinforcement Learning

Offline reinforcement learning (RL) extends the paradigm of classical RL algorithms to purely learning from static datasets, without interacting with the underlying environment during the learning process. A key challenge of offline RL is the instability of policy training, caused by the mismatch between the distribution of the offline data and the undiscounted stationary state-action distribution of the learned policy. To avoid the detrimental impact of distribution mismatch, we regularize the undiscounted stationary distribution of the current policy towards the offline data during the policy optimization process. Further, we train a dynamics model to both implement this regularization and better estimate the stationary distribution of the current policy, reducing the error induced by distribution mismatch. On a wide range of continuous-control offline RL datasets, our method indicates competitive performance, which validates our algorithm. The code is publicly available.

==> Tex/theory.tex <==
\subsection{Model-Based Joint Matching}

we denote the true transition model as $ P^{*}$, and the
model we learn as $\widehat{P}.$ 
We denote $d_{\denv}$ as the state-action distribution in the offline dataset $\denv$.
Then for the integral probabiliity metric $D_{\gG}$ and the current policy $\pi$ we have 

\begin{equation*}
    D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\denv}}\leq {D_{\gG}}\br{d_{\pi}^{\widehat{P}},d_{\denv}}+D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}}.
\end{equation*}

The first term we can use similar idea as joint matching to have a
computational regularization, and for the second term, we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & :=\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & :=\sup_{g\in\mathcal{G}}\abs{\mathrm{GAP}(s,a)}
\end{align*}

\begin{align*}
\mathrm{GAP}(s,a) & =(1-\gamma)\mathbb{E}_{s\sim \mu_{0},a\sim\pi}\left[\widehat{Q}^{\pi}(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\\
 & =-\gamma\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot \given s,a),a^{\prime}\sim\pi(\cdot\given s^{\prime})}\left[\widehat{Q}^{\pi}(s^{\prime},a^{\prime})\right]+\gamma\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim\widehat{P}(\cdot\given s, a),a^{\prime}\sim\pi(\cdot\given s ^{\prime})}\left[\widehat{Q}^{\pi}(s^{\prime},a^{\prime})\right]\\
 & =-\gamma\left(\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]\right]\right)\\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[D_{\mathrm{TV}}\left(P^{*}(s^{\prime}\given s,a)\Vert\widehat{P}(s^{\prime}\given s,a)\right)\right]\\
\end{align*}

The problem is that we can not get the sample from $d_{\pi}^{ P^{*}}(s,a)$.
Denote $\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)=D_{\mathrm{TV}}\left(P^{*}(s^{\prime}\given s,a)\Vert\widehat{P}(s^{\prime}\given s,a)\right)$,
then we have 

\begin{align*}
\mathrm{GAP}(s,a) & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathcal{\mathbb{E}}_{(s,a)\sim\denv}\left[\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)\right]+\frac{2\gamma g_{\max}}{1-\gamma}\int\left(\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)\left(d_{\denv}(s,a)-d_{\pi}^{ P^{*}}(s,a)\right)dads\right)\\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim\denv}\sqrt{\frac{1}{2}\mathrm{KL}\br{P^*\Vert\widehat{P}}}+\frac{2\gamma g_{\max}M}{1-\gamma}\int\left(\frac{1}{M}\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)\left(d_{\denv}(s,a)-d_{\pi}^{ P^{*}}(s,a)\right)dads\right)\\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim\denv}\sqrt{\frac{1}{2}\mathrm{KL}\br{P^*\Vert\widehat{P}}}+\frac{2\gamma g_{\max}M}{1-\gamma}\sup_{f\in\mathcal{F}}\left\vert f(s,a)\left(d_{\denv}(s,a)-d_{\pi}^{ P^{*}}(s,a)\right)\right\vert \\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim\denv}\sqrt{\frac{1}{2}\mathrm{KL}\br{P^*\Vert\widehat{P}}}+\frac{2\gamma g_{\max}M}{1-\gamma} D_{\mathcal{F}}\left(d_{\denv}(s,a),d_{\pi}^{P^{*}}(s,a)\right)
\end{align*}

Similarly using the change of variable trick, the last term becomes 

\begin{align*}
D_{\mathcal{F}}\left(d_{\denv}(s,a), d_{\pi}^{P^*}(s,a)\right) & :=\sup_{f\in\mathcal{F}}\left\vert \mathbb{E}_{(s,a)\sim\denv}\left[f(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{P^*}(s,a)}[f(s,a)]\right\vert \\
 & =\sup_{Q_{f}\in\mathcal{\mathcal{Q}}}\left\vert \mathbb{E}_{(s,a,s^{\prime})\sim\denv,a^{\prime}\sim\pi}\left[Q_{f}(s,a)-\gamma Q_{f}\br{s^{\prime},a^{\prime}}\right]-(1-\gamma)\mathbb{E}_{s\sim \mu_{0},a\sim\pi}\left[Q_{f}(s,a)\right]\right\vert \\
\end{align*}

\subsection{Model-based Joint Matching: Average Case}

we denote the true transition model as $ P^{*}$, and the
model we learnt by maximizing likelihood as $\widehat{P}$.
We denote $d_{\denv}$ as the state-action distribution in the offline dataset $\denv$ and $\pi$ as the current policy.
Then we have 
\begin{equation*}
    D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\denv}}\leq D_{\gG}\br{d_{\pi}^{\widehat{P}},d_{\denv}}+D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}},
\end{equation*}
where the first term is the one we used for optimizing policy. According
to previous change of variable trick, we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{\widehat{P}},d_{\denv}} & :=\text{\ensuremath{\sup_{g\in\mathcal{G}}\abs{\mathbb{E}_{(s,a)\sim\denv}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim\denv,s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[g(s^{\prime},a^{\prime})\right]}\text{}.}}\\
\end{align*}

In practice we can rollout more than 1 step to increase the efficiency
of the model. 

For the second term $D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}}$,
we have 
\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & :=\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
\end{align*}

Define $\widehat{V}^{\pi}(s)$ and $\widehat{Q}^{\pi}(s)$ as the value and
state action value function induced by policy $\pi$ and the learned
transition model $\widehat{P}(s^{\prime}\given s,a)$, then we have
the average Bellman equation

\[
\widehat{\eta}^{\pi}=\lim_{T\to\infty}\mathbb{E}_{\tau\sim p_{\pi}}\left[\frac{1}{T+1}\sum_{t=0}^{\infty}r_{t}\right]=\mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]
\]
\begin{align*}
\widehat{Q}^{\pi}(s,a)-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right] & =g(s,a)-\widehat{\eta}^{\pi}\,,\\
\end{align*}

Then we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & :=\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert \widehat{\eta}^{\pi}-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot\given s ,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)-g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert -\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)-g(s,a)+\widehat{\eta}^{\pi}\right]\right\vert \\
 & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert -\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat V^{\pi}(s^{\prime})\right]\right]\right\vert \\
 & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat V^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat V^{\pi}(s^{\prime})\right]\right]\right\vert \\
\end{align*}

If we define $\mathcal{E}\br{s,a;\widehat{V}^{\pi}}:=\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s ,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]$,
and assume $\sup_{\widehat V^\pi \in \gV} \norm{\widehat V^\pi}_{\infty} \leq V_{\mathrm{max}}$, then we know 

\begin{align*}
\mathcal{E}\br{s,a;\widehat{V}^{\pi}} & :=\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]\\
 & =\int\left( P^{*}(\cdot\given s,a)-\widehat{P}(\cdot\given s,a)\right)\widehat{V}^{\pi}\br{s^{\prime}}ds^{\prime}\\
 & \leq V_{\max}\int\left\vert  P^{*}(\cdot\given s,a)-\widehat{P}(\cdot\given s,a)\right\vert ds^{\prime}\\
 & \leq2V_{\max}\,.
\end{align*}

Recall that the total variation distance is a special instance of the integral probability metrics $D_\gG$ when the function class $\gG = \cbr{g: \norm{g}_\infty \leq 1}$ \citep{ipm2009,mmdgangp2018}.

Then we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathcal{E}\br{s,a,\widehat{V}^{\pi}}\right]\right\vert \\
 & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\denv}}\left[\mathcal{E}\br{s,a,\widehat{V}^{\pi}}\right]+\int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}(s,a)-d_{\denv}(s,a)\right)dads\right\vert \\
 & \leq\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\denv}}\left[\mathcal{E}\br{s,a,\widehat{V}^{\pi}}\right]\right\vert +\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}(s,a)-d_{\denv}(s,a)\right)dads\right\vert \\
 &\leq \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathcal{E}\br{s,a,\widehat{V}^{\pi}} \right\vert \right]  + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}(s,a)-d_{\denv}(s,a)\right)dads\right\vert \\
 &= V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{s^{\prime}\sim P^{*}}\left[\frac{\widehat{V}^{\pi}(s^{\prime})}{V_{\mathrm{max}}}\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}}\left[\frac{\widehat{V}^{\pi}(s^{\prime})}{V_{\mathrm{max}}}\right]
 \right\vert \right] + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}-d_{\denv}\right)dads\right\vert \\
 &= V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \mathrm{TV}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)} \right] + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}-d_{\denv}\right)dads\right\vert \\
 &\leq V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sqrt{{1 \over 2} \mathrm{KL}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)}} \right] + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}-d_{\denv}\right)dads\right\vert
\end{align*}
since $\norm{\frac{\widehat{V}^{\pi}}{V_{\mathrm{max}}}}_\infty \leq 1$, where we use Lemma~\ref{thm:lemma_exchange_sup_exp} to exchange order between $\sup$ and $\E[\cdot]$, and the last bound is from the Pinsker's inequality. 
The first term of the last equation can be minimize via the maximum likelihood estimation on $\widehat P$ since 
\begin{equation*}
    \begin{split}
        & \min_{\widehat P} V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sqrt{{1 \over 2} \mathrm{KL}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)}} \right] \\
        \leq&  \min_{\widehat P}  V_{\mathrm{max}}  \sqrt{{1 \over 2} \mathbb{E}_{(s,a)\sim d_{\denv}} \sbr{\mathrm{KL}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)}}}  \\
        =&  \min_{\widehat P} V_{\mathrm{max}} \sqrt{{1\over 2} \mathbb{E}_{(s,a)\sim d_{\denv}}\sbr{\int P^*(s' \given s,a)\br{\log P^*(s' \given s,a) - \log \widehat P(s' \given s,a)} ds'}} \\
        =&  \min_{\widehat P} V_{\mathrm{max}} \sqrt{{1\over 2} \cbr{\mathbb{E}_{(s,a)\sim d_{\denv}}\sbr{\int P^*(s' \given s,a) \log P^*(s' \given s,a) ds'} - \mathbb{E}_{(s,a)\sim d_{\denv}} \sbr{\int P^*(s' \given s,a)\log \widehat P(s' \given s,a) ds'}}}    
        \\ =&  V_{\mathrm{max}} \sqrt{ {1\over 2} \cbr{\mathbb{E}_{(s,a,s')\sim d_{\denv}}\sbr{ \log P^*(s' \given s,a) } + \min_{\widehat P} \cbr{- \mathbb{E}_{(s,a,s')\sim d_{\denv}} \sbr{ \log \widehat P(s' \given s,a)}}}},
    \end{split}
\end{equation*}
where $V_{\mathrm{max}}$ is a constant and the first term inside $\sqrt{\cdot}$ is a constant, and 
\begin{equation*}
    \arg \min_{\widehat P} \cbr{- \mathbb{E}_{(s,a,s')\sim d_{\denv}} \sbr{ \log \widehat P(s' \given s,a)}} = \arg \max_{\widehat P}  \mathbb{E}_{(s,a,s')\sim d_{\denv}} \sbr{ \log \widehat P(s' \given s,a)}
\end{equation*}
which is exactly the model-training objective Equation~\eqref{eq:model_objective}.


==> icml 2022_joint_matching_model_base/Tex/background.tex <==
\section{Background} \label{sec:background}

% RL
We follow the classical RL setting \citep{rlintro2018} to model the interaction between the agent and the environment as a Markov Decision Process (MDP), specified by the tuple $\gM = \br{\sS, \sA, P, r, \gamma, \mu_0}$, where $\sS$ denotes the state space, $\sA$ the action space, $P\br{s' \given s, a}: \sS \times \sS \times \sA \rightarrow [0,1]$ the environmental dynamic, $r(s,a): \sS \times \sA \rightarrow [-r_{max}, r_{max}]$ the reward function, $\gamma \in (0,1]$ the discount factor, and $\mu_0(s): \sS \rightarrow [0,1]$ the initial-state distribution.

% OPE (def of both discounted and undiscounted distribution)
For a given policy $\pi(a\given s)$, we follow the literature \citep{markovdp1994,breakingcurse2018}
to denote the state-action distribution at timestep $t \geq 0$ induced by policy $\pi$ on MDP $\gM$ as 
$
 d_{\pi, t}(s,a) :=  \Pr\br{s_t = s, a_t = a \given s_0 \sim \mu_0, a_t \sim \pi, s_{t+1} \sim P,\forall\, t \geq 0}.
$
Denote the \textit{discounted} stationary state-action distribution induced by $\pi$ as
$
    d_{\pi,\gamma}(s,a) = (1 - \gamma) \sum_{t=0}^\infty \gamma^t d_{\pi, t}(s,a)
$
and the \textit{undiscounted (average)} stationary state-action distribution as $d_\pi(s,a) = \lim_{T \rightarrow \infty}\sum_{t=0}^T \frac{1}{T+1} d_{\pi, t}(s,a)$.
We have $d_{\pi,\gamma}(s,a) = d_{\pi,\gamma}(s) \pi(a \given s)$ and $d_\pi(s,a) = d_\pi(s) \pi(a \given s)$.
% offline RL background
In offline RL \citep{offlinetutorial2020}, one has only access to a static dataset $\denv = \cbr{(s,a,r,s')}$ collected by some behavior policy $\pi_b$, which can be a mixture of several data-collecting policies.

% Actor-Critic Algorithm (def of Q, training of Q, training of \pi)
Denote the action-value function for policy $\pi$ on $\gM$ as $Q^\pi(s,a) = \E_{\pi, P, r}\sbr{\sum_{t=0}^\infty \gamma^t r(s_t,a_t) \given s_0 = s, a_0 = a}$.
In the actor-critic algorithm \citep{rlintro2018}, the policy $\pi$ and critic $Q^\pi(s,a)$ are typically modelled as parametric functions $\pi_\vphi$ and $Q_\vtheta$,  parametrized by $\vphi$ and $\vtheta$, respectively.
In offline RL, the critic is trained in the policy evaluation step by Bellman backup as minimizing {\it w.r.t.} $\vtheta$:
% \begin{equation}\textstyle \label{eq:ac_bellman}
% \resizebox{.48\textwidth}{!}{%
% $
%     \E_{(s,a,s')\sim \denv} \sbr{\br{Q_{\vtheta}(s, a) - \br{ r(s, a) + \gamma \E_{\, a' \sim \pi(\cdot \given s')} \sbr{Q_{\vtheta}(s', a')}}}^2};
% $%    
% }
% \end{equation}
\begin{align}
    &\ell(\vtheta):= \E_{(s,a,r,s')\sim \denv} \left[\left(Q_{\vtheta}(s,a)  - \hat{B}^\pi Q_{\vtheta^\prime}(s,a)\right)^2\right]\,,\notag \\ 
    &\hat{B}^\pi Q_{\vtheta^\prime}(s,a)= r(s,a) + \gamma \E_{a^\prime\sim \pi(\cdot  \given s^\prime)}\left[Q_{\vtheta^\prime}(s^\prime, a^\prime)\right]\,, \label{eq:ac_bellman}
\end{align}
where $Q_{\vtheta^\prime}$ is the target network. 
The actor $\pi_\vphi$ is trained in the policy improvement step as
\begin{equation}\textstyle \label{eq:ac_actor}
     \arg\max_\vphi \E_{s \sim d_{\pi_b}(s),\, a \sim \pi_{\vphi}(\cdot \given s)}\sbr{Q_{\vtheta}\br{s, a}},
\end{equation}
where samples from the offline dataset $\denv$ is used to approximate the samples from $d_{\pi_b}(s)$ \citep{diagbottleneck2019, offlinetutorial2020}.

% model-based RL
In model-based offline RL, a stochastic dynamic model $\widehat P\br{s' \given s, a}$ within some function class $\mathcal{P}$ is learned to approximate the true environmental dynamic, denoted as $P^*$.
With the offline dataset $\denv$, $\widehat P$ is typically trained using MLE \citep{mbpo2019, mopo2020, combo2021}  as
\begin{equation}\textstyle \label{eq:model_objective}
    \arg\max_{\widehat P \in \mathcal{P}} \E_{\br{s,a,s'} \sim \denv}\sbr{\log \widehat P\br{s' \given s, a}}.
\end{equation}
Models for the reward function $\hat r$ and the termination conditional can also be trained similarly if assumed unknown.
With $\widehat P$ and $\hat r$, an approximated MDP to $\gM$ can be constructed as $\widehat \gM = (\sS, \sA, \widehat P, \hat r, \gamma, \mu_0)$.
To distinguish the aforementioned stationary distributions induced by policy $\pi$ on $\gM$ and on $\widehat \gM$, we denote the undiscounted stationary state-action distribution induced by $\pi$ on the true dynamic $P^*$ (or $\gM$) as $d_\pi^{P^*}(s,a)$, on the learned dynamic $\widehat P$ (or $\widehat M$) as $d_\pi^{\widehat P}(s,a)$, and similarly for the discounted stationary state-action distributions $d_{\pi,\gamma}^{P^*}(s,a)$ and $d_{\pi,\gamma}^{\widehat P}(s,a)$.
With the estimated dynamic $\widehat P$, prior model-based offline RL works \citep{morel2020,mopo2020,combo2021,mabe2021} typically approximate $d_{\pi_\vphi}^{P^*}(s,a)$ by simulating the learned policy $\pi_\vphi$ in $\widehat M$ for a short horizon $h$ starting from state $s \in \denv$.
The resulting trajectories are stored into a replay buffer $\dmodel$, similar to the replay buffer in off-policy RL \citep{replaybuffer1992,ddpg2016}.
Sampling from $\denv$ in Eqs.~\eqref{eq:ac_bellman} and \eqref{eq:ac_actor} is commonly replaced by sampling from the augmented dataset $\mathcal{D} := f \denv + (1-f) \dmodel, f \in [0,1]$, denoting  sampling from $\denv$ with probability $f$ and from $\dmodel$ with probability $1 - f$.

We follow the offline RL literature \citep{breakingcurse2018, algaedice2019, confoundingrobust2020,gendice2020} to assume
\textbf{(i)} that all the Markov chains induced by the studied (approximated) dynamics and policies are ergodic, and thus the undiscounted stationary state-action distribution $d_\pi(s,a)$ equals to the limiting state-action occupancy measure induced by $\pi$ on the corresponding MDP;
and \textbf{(ii)} that the offline dataset $\denv$ is constructed as the rollouts of $\pi_b$ on the true dynamic $P^*$, \textit{i.e.}, $\denv \sim d_{\pi_b}^{P^*}(s,a)$.
We denote the state-action and state distributions in $\denv$ as $d_{\denv}(s,a)$ and $d_{\denv}(s)$, which are  discrete approximations to $d_{\pi_b}^{P ^*}(s,a)$ and $d_{\pi_b}^{P ^*}(s)$, respectively.



==> icml 2022_joint_matching_model_base/Tex/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
In this paper, we directly approach a central difficulty in offline RL, {\it i.e.}, the mismatch between the distribution of the offline dataset and the undiscounted stationary state-action distribution of the learned policy.
Specifically, we derive a tractable bound for the difference between the stationary distribution of the behavior policy in the underlying environmental dynamic and that of the learned policy {\it w.r.t.} the IPM.
Based on the theoretical derivation, we design a practical model-based algorithm that uses this tractable bound as a regularizer in the policy improvement step.
Our practical implementation is tested on a diverse array of continuous-control offline-RL datasets and shows competitive performance compared with several state-of-the-art model-based and model-free baselines.
Ablation study is also provided to validate some of the key algorithmic choices.

\section*{Acknowledgements}
The authors acknowledge the support of NSF IIS1812699 and ECCS-1952193, the support of a gift fund from ByteDance
Inc., and the Texas Advanced Computing Center (TACC)
for providing HPC resources that have contributed to the
research results reported within this paper.

==> icml 2022_joint_matching_model_base/Tex/exp.tex <==
\section{Experiments} \label{sec:experiment}
\begin{figure}[t]
     % \vspace{+2mm}
     \centering
     \begin{subfigure}[b]{0.11\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/true_testset.pdf}
         \caption{Truth}
         \label{fig:toy_truth}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/DGAN-1-iter_100000.pdf}
         \caption{D-CGAN}
         \label{fig:toy_dcgan}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/GGAN-1-iter_100000.pdf}
         \caption{G-CGAN}
         \label{fig:toy_gcgan}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/CGAN-1-iter_100000.pdf}
         \caption{CGAN}
         \label{fig:toy_cgan}
     \end{subfigure}
     \vspace{-3mm}
        \caption{ 
        Performance of approximating the behavior policy on the circle dataset. 
        A deterministic-generator conditional GAN (``D-CGAN"), a Gaussian-generator conditional GAN (“G-CGAN”) and a conditional GAN (``CGAN") are fitted using the classical policy (conditional distribution) matching approach similar to \citet{brac2019}.
        More details are provided in Appendix \ref{sec:toy_details}.
        }
        \label{fig:toy}
        \vspace{-6.5mm}
\end{figure}

In what follows, we first show the effectiveness of an implicit policy through a toy example (\Secref{sec:exp_toy}).
We then present an empirical evaluation of our algorithm (\Secref{sec:exp_main}), followed by an ablation study (\Secref{sec:exp_ablation}).
{Source code for the experiments is publicly \href{https://github.com/Shentao-YANG/SDM-GAN_ICML2022}{available}.}

%\yf{make the figure smaller, it is too alarge and has too much space}

\subsection{Toy Experiments}\label{sec:exp_toy}


As a motivation to train a flexible implicit policy instead of the classical deterministic or Gaussian policy, we conduct a toy behavior-cloning experiment, as shown on Figure~\ref{fig:toy}.
We remark that the simplest form of offline behavior cloning is essentially a supervised learning task, with the reward function and the termination condition being unnecessary.
Throughout Figure~\ref{fig:toy}, we use the $x$-axis to represent the state and $y$-axis the action.
Figure~\ref{fig:toy_truth} plots the state-action distribution that we seek to clone, which presents multimodality on almost all states.
Such an offline dataset may come from multiple data-collecting policies or from the multiple maxima of the action-value function on the action space.
We hence expect the learned policy to capture the targeted state-action distribution, which can translate into a better capture of the rewarding actions and an improved generalization beyond the static dataset in offline RL tasks.
Figures~\ref{fig:toy_dcgan}-\ref{fig:toy_cgan} plot the state-action distributions of the learned policies on the testset, in which we compare the implicit policy implemented by conditional GAN (Figure~\ref{fig:toy_cgan}) with its variants of changing the implicit generator to deterministic transformation (Figure~\ref{fig:toy_dcgan}) and to the Gaussian generator (Figure~\ref{fig:toy_gcgan}).
Experimental details are discussed in Appendix~\ref{sec:toy_details}.

We see from Figures~\ref{fig:toy_dcgan} and \ref{fig:toy_gcgan} that both the deterministic and the Gaussian policy fail to capture necessary action modes, which directly relates to their less flexible structures.
By contrast, as shown in Figure~\ref{fig:toy_cgan}, the implicit policy defined by conditional GAN does capture all the action modes on each state and fits well onto the targeted distribution.
This toy example motivates our algorithmic design of training an implicit policy via the conditional GAN structure.

\subsection{Main Results}\label{sec:exp_main}
\begin{table*}[h] 
 \vspace{-1mm}
\caption{
Normalized returns for the experiments on the D4RL datasets.
We use the ``v0” version of the datasets in the Gym-MuJoCo and Adroit domains.
On the Gym-Mojoco domain, we bold both the highest score over all algorithms and the highest score of model-based  algorithms. 
On the Maze2D and Adroit tasks, we bold the best scores. 
} 
\label{table:main} 
\centering 
\def\arraystretch{1.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
                 Task Name &  aDICE &                               CQL &                        FisherBRC &                           TD3+BC &                          OptiDICE &                                     MOPO &                                    COMBO &                                WMOPO &                           SDM-GAN \\
\midrule
        halfcheetah-medium &   -2.2 &    39.0 $\pm$ {\footnotesize 0.8} &   41.1 $\pm$ {\footnotesize 0.6} &   43.0 $\pm$ {\footnotesize 0.5} &    38.2 $\pm$ {\footnotesize 0.5} &           47.2 $\pm$ {\footnotesize 1.0} &           53.7 $\pm$ {\footnotesize 2.1} &           \textbf{55.6} $\pm$ {\footnotesize 1.3} &    42.5 $\pm$ {\footnotesize 0.5} \\
           walker2d-medium &    0.3 &   60.2 $\pm$ {\footnotesize 30.8} &   \textbf{78.4} $\pm$ {\footnotesize 1.8} &   77.3 $\pm$ {\footnotesize 4.0} &   14.3 $\pm$ {\footnotesize 15.0} &            0.0 $\pm$ {\footnotesize 0.1} &          40.9 $\pm$ {\footnotesize 28.9} &          22.7 $\pm$ {\footnotesize 27.7} &    \textbf{66.7} $\pm$ {\footnotesize 1.8} \\
             hopper-medium &    1.2 &   34.5 $\pm$ {\footnotesize 11.7} &   99.2 $\pm$ {\footnotesize 0.3} &   \textbf{99.6} $\pm$ {\footnotesize 0.6} &   92.3 $\pm$ {\footnotesize 16.9} &           23.4 $\pm$ {\footnotesize 7.2} &          51.8 $\pm$ {\footnotesize 32.8} &          \textbf{66.5} $\pm$ {\footnotesize 46.0} &   62.8 $\pm$ {\footnotesize 14.3} \\
 halfcheetah-medium-replay &   -2.1 &    43.4 $\pm$ {\footnotesize 0.8} &   43.2 $\pm$ {\footnotesize 1.3} &   41.9 $\pm$ {\footnotesize 2.0} &    39.8 $\pm$ {\footnotesize 0.8} &           \textbf{52.5} $\pm$ {\footnotesize 1.4} &           51.8 $\pm$ {\footnotesize 1.6} &           51.8 $\pm$ {\footnotesize 5.6} &    41.7 $\pm$ {\footnotesize 0.4} \\
    walker2d-medium-replay &    0.6 &    16.4 $\pm$ {\footnotesize 6.6} &  38.4 $\pm$ {\footnotesize 16.6} &   24.6 $\pm$ {\footnotesize 6.7} &    20.2 $\pm$ {\footnotesize 5.8} &          51.9 $\pm$ {\footnotesize 15.8} &          14.2 $\pm$ {\footnotesize 11.9} &          \textbf{54.8} $\pm$ {\footnotesize 12.3} &    20.3 $\pm$ {\footnotesize 4.0} \\
      hopper-medium-replay &    1.1 &    29.5 $\pm$ {\footnotesize 2.3} &   33.4 $\pm$ {\footnotesize 2.8} &   31.4 $\pm$ {\footnotesize 2.7} &    29.0 $\pm$ {\footnotesize 4.9} &          47.1 $\pm$ {\footnotesize 16.2} &           34.5 $\pm$ {\footnotesize 2.0} &           \textbf{93.9} $\pm$ {\footnotesize 1.9} &    30.6 $\pm$ {\footnotesize 2.8} \\
 halfcheetah-medium-expert &   -0.8 &   34.5 $\pm$ {\footnotesize 15.8} &   \textbf{92.5} $\pm$ {\footnotesize 8.5} &   90.1 $\pm$ {\footnotesize 6.9} &   91.2 $\pm$ {\footnotesize 16.6} &           \textbf{92.1} $\pm$ {\footnotesize 8.3} &          90.0 $\pm$ {\footnotesize 10.5} &          42.7 $\pm$ {\footnotesize 13.0} &    89.1 $\pm$ {\footnotesize 6.6} \\
    walker2d-medium-expert &    0.4 &   79.8 $\pm$ {\footnotesize 22.7} &  \textbf{98.2} $\pm$ {\footnotesize 13.1} &  96.1 $\pm$ {\footnotesize 15.8} &   67.1 $\pm$ {\footnotesize 30.2} &          36.0 $\pm$ {\footnotesize 49.6} &          61.3 $\pm$ {\footnotesize 36.1} &          48.6 $\pm$ {\footnotesize 37.0} &    \textbf{97.9} $\pm$ {\footnotesize 4.9} \\
      hopper-medium-expert &    1.1 &  103.5 $\pm$ {\footnotesize 20.2} &  112.3 $\pm$ {\footnotesize 0.3} &  111.9 $\pm$ {\footnotesize 0.3} &  101.8 $\pm$ {\footnotesize 18.5} &           27.8 $\pm$ {\footnotesize 3.6} &          \textbf{112.6} $\pm$ {\footnotesize 1.8} &          97.8 $\pm$ {\footnotesize 19.3} &   104.5 $\pm$ {\footnotesize 5.4} \\
              maze2d-large &   -0.1 &   43.7 $\pm$ {\footnotesize 18.6} &   -2.1 $\pm$ {\footnotesize 0.4} &  87.6 $\pm$ {\footnotesize 15.4} &  130.7 $\pm$ {\footnotesize 56.1} &  - &  - &  - &  \textbf{207.7} $\pm$ {\footnotesize 11.7} \\
             maze2d-medium &   10.0 &    30.7 $\pm$ {\footnotesize 9.8} &   4.6 $\pm$ {\footnotesize 20.4} &  59.1 $\pm$ {\footnotesize 47.7} &  \textbf{140.8} $\pm$ {\footnotesize 44.0} &  - &  - &  - &  115.4 $\pm$ {\footnotesize 34.2} \\
              maze2d-umaze &  -15.7 &    50.5 $\pm$ {\footnotesize 7.9} &  -2.3 $\pm$ {\footnotesize 17.9} &  13.8 $\pm$ {\footnotesize 22.8} &  \textbf{107.6} $\pm$ {\footnotesize 33.1} &  - &  - &  - &   36.1 $\pm$ {\footnotesize 28.4} \\
                 pen-human &   -3.3 &    2.1 $\pm$ {\footnotesize 13.7} &    0.0 $\pm$ {\footnotesize 3.9} &   -1.7 $\pm$ {\footnotesize 3.8} &    -0.1 $\pm$ {\footnotesize 5.6} &  - &  - &  - &    \textbf{17.8} $\pm$ {\footnotesize 1.7} \\
                pen-cloned &   -2.9 &     1.5 $\pm$ {\footnotesize 6.2} &   -2.0 $\pm$ {\footnotesize 0.8} &   -2.4 $\pm$ {\footnotesize 1.4} &     1.4 $\pm$ {\footnotesize 6.8} &  - &  - &  - &    \textbf{40.6} $\pm$ {\footnotesize 6.1} \\
                pen-expert &   -3.5 &   95.9 $\pm$ {\footnotesize 18.1} &  31.6 $\pm$ {\footnotesize 24.4} &  32.4 $\pm$ {\footnotesize 24.3} &    -1.1 $\pm$ {\footnotesize 4.7} &  - &  - &  - &  \textbf{135.8} $\pm$ {\footnotesize 11.7} \\
               door-expert &    0.0 &   87.9 $\pm$ {\footnotesize 21.6} &  57.6 $\pm$ {\footnotesize 37.7} &   -0.3 $\pm$ {\footnotesize 0.0} &   87.9 $\pm$ {\footnotesize 25.8} &  - &  - &  - &    \textbf{93.5} $\pm$ {\footnotesize 6.7} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table*}

%\yf{Can we add some summary paragraph textbf? it is a little bit too long for readers}
As discussed in \Secref{sec:main_method_details}, we implement our algorithm by approximately matching the JSD between the stationary distributions via the conditional GAN, which we dub as Stationary Distribution Matching via GAN (SDM-GAN).
We compare our algorithm with three state-of-the-art (SOTA) model-free offline-RL algorithms: CQL \citep{cql2020}, FisherBRC \citep{fisherbrc2021}, and TD3+BC \citep{td3bc2021}; three SOTA model-based offline-RL algorithms: MOPO \citep{mopo2020}, COMBO \citep{combo2021}, and WMOPO \citep{wmopo2021};
{and two ``DICE-style" algorithms: AlgaeDICE \citep{algaedice2019} and OptiDICE \citep{optidice2021}}.
For WMOPO, we use the version of $\alpha = 0.2$, which is the paper's proposal.
Experimental details and hyperparameter setups are discussed in detail in Appendix~\ref{sec:rl_exp_details}.
We remark that unlike our algorithm, the three model-based RL baselines assume known termination function and possibly also known reward function, which potentially limits their applicability.
% rerun the result
{
Except AlgaeDICE, we rerun each baseline method using the official source code under the recommended hyperparameters.
The results of AlgaeDICE (``aDICE") is obtained from the D4RL whitepaper \citep{fu2021d4rl}.
}
% three domain of tasks, mbrl do not have maze2d and adroit
We compare our algorithm with the baselines on a diverse set of continuous-control offline-RL datasets (discussed in detail in Appendix~\ref{sec:rl_exp_details}), ranging across the Gym-Mojoco, Maze2D, and Adroit domains in the D4RL benchmark.
Note that the three model-based RL baselines do not provide hyperparameter configurations for the Maze2D and Adroit domains, and therefore we do not evaluate them on these datasets.
Table~\ref{table:main} shows the mean and standard deviation of each algorithm on each tested dataset.

In Table~\ref{table:main}, our algorithm shows competitive and relatively-stable performance across a diverse array of datasets.
Specifically, compared to the baselines, our algorithm shows better and more robust performance on the two task domains that are traditionally considered as challenging in offline-RL  \citep{fu2021d4rl}: 
the Adroit domain featured by high dimensionality and narrow data-distribution; and the Maze2D domain collected by non-Markovian policies.
On these two domains, behavioral-cloning (BC) based algorithms, such as FisherBRC and TD3+BC, are likely to fail. 
Concretely, on the Adroit datasets, a main difficulty is estimating the behavior policy and regularizing the current policy towards it in a high-dimensional space with limited data. 
On the Maze2D datasets, policy learning is challenged by the error of using a Markovian policy to clone the non-Markovian data-collecting policy.
The complexity of these datasets and underlying environments may also call for a more flexible policy class, and thus excels our design of an implicit policy over the classical deterministic or Gaussian policy.
On the Gym-Mojoco domain, our algorithm is able to learn from median-quality datasets and from samples collected by a mixture of data-collecting policies, which are closer to the real-world settings.

{
Comparing SDM-GAN with AlgaeDICE and OptiDICE reveals the overall benefit of our approach over the ``DICE-style" method.
As an example, OptiDICE requires BC, which is implemented by a Gaussian-mixture policy with several components.
While this BC strategy may be beneficial on relatively-lower dimensional Maze2D datasets, it may not generalize onto the higher-dimensional Adroit datasets. 
This may be a direct result of the previously-stated difficulty of BC-based methods on the Adroit datasets.
}

Additionally, we notice that some of the designs in these SOTA baselines are orthogonal to our algorithm, such as a tactful estimation of the action-value function (CQL, FisherBRC, COMBO), an incorporation of uncertainty quantification into the estimated dynamic (MOPO), and a density-ratio-based weighted model estimation (WMOPO).
These designs may be easily incorporated into our algorithm, leaving future work and potentials for further improvement.
% We leave such an investigation for future work.

\subsection{Ablation Study} \label{sec:exp_ablation}

\begin{figure*}[ht]
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/compare_f_0508.pdf}
        %  \vspace{-7mm}
         \caption{Varying $f \in \cbr{0, 0.05, 0.5, 0.8, 1}$}
         \label{fig:varying_f}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/compare_alpha.pdf}
         \caption{Varying $\alpha \in \cbr{2.5, 10, 25}$ and No Reg.}
         \label{fig:varying_alpha}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/compare_with_w1.pdf}
         \caption{JSD {\it v.s.} IPM (Wasserstein-$1$ Dual)}
         \label{fig:jsd_imp}
     \end{subfigure}
     \vspace{-8mm}
        \caption{ 
        Average score ($x$-axis) over the tested datasets for each of the comparison in the ablation study (\Secref{sec:exp_ablation}).
        }
        \label{fig:ablation}
        \vspace{-6mm}
\end{figure*}

In the ablation study we seek to answer the following questions:
\textbf{(a)} Does the rollout dataset $\dmodel$ help the performance?
\textbf{(b)} Is our algorithm sensitive to the choice of the regularization coefficient $\alpha$?
\textbf{(c)} Does approximately matching the JSD between the stationary distributions perform better than matching the IPM?
Unless stated otherwise, experimental details for all algorithmic variants follow the main results (stated in Appendix~\ref{sec:rl_exp_details}).

\textbf{(a).} To investigate whether rollout data are helpful for policy training, we follow \citet{combo2021} to compare our algorithm used in \Secref{sec:exp_main} ($f=0.5$) with its variant of fewer and more rollout data, respectively $f=0.8$ and $f=0.05$, with all other settings kept the same.
{Additionally, we consider the variants of no rollout data ($f=1$) and only rollout data ($f=0$).}

Figure~\ref{fig:varying_f} plots the average score over the tested datasets for each variant, with detail comparison provided in Table~\ref{table:f_0508}.
On $11$ out of $16$ datasets, the $f=0.5$ version has higher mean returns than the $f=0.8$ version, showing the efficacy of using more rollout data.
This empirical result aligns with our intuition that rollout data can better approximate the stationary state-action distribution of the learned policy, especially when the learned policy  deviates from the behavior.
{The efficacy of model-based rollout is further corroborated by the generally worse performance of the $f=1$ variant, compared with $f=0.8$ and $f=0.5$.
Nevertheless, using too-many rollout data can be harmful, as shown by the comparison between the $f=0$, $f=0.05$, and $f=0.5$ variants.
In Table~\ref{table:f_0508}, the scores for the $f=0$ and $f=0.05$ variants are generally lower than $f=0.5$, and the standard deviations relative to the scores are generally higher.
This comparison shows the gain of adding offline data for combating the inaccuracy in the estimated dynamic.}
% This is likely due to the inaccuracy in the estimated dynamics.

\textbf{(b).} 
We test our algorithm on both a smaller and a larger value of the regularization coefficient $\alpha \in \cbr{2.5, 25}$, {together with the variant without the proposed regularization term (denoted as ``No Reg.")}.
Figure~\ref{fig:varying_alpha} plots the average scores and Table~\ref{table:alpha_sweep} presents the results.
We see that on a large portion of datasets, our method is relatively robust to the choice of $\alpha$, especially when using a larger value of $\alpha$.

A small value of $\alpha$, \textit{e.g.}, $\alpha=2.5$ in \citet{td3bc2021}, can be too conservative for our algorithm, limiting the improvement of the policy.
A larger value of $\alpha=25$, which puts more weight on policy optimization than the default $\alpha=10$, overall does not lead to significant deterioration in the performance, though the results do in general possess higher variance.
{
The inferior performance of the ``No Reg." variant shows the necessity of proper regularization, especially on the Maze2D and Adroit datasets. 
}

\textbf{(c).} 
We compare our default algorithm of approximately matching the JSD between the stationary distributions (SDM-GAN) with the variant of approximately matching the dual form of the Wasserstein-$1$ metric, which is an instance of the IPM \citep{ipm1997,ipm2009} and is dubbed as ``SDM-WGAN.''
SDM-WGAN is implemented by changing the CGAN structure in SDM-GAN with the WGAN-GP structure \citep{wgangp2017}.
We vary the strength of the Lipschitz-$1$ constraint $\lambda_{\mathrm{GP}}$ in WGAN-GP over $\lambda_{\mathrm{GP}} \in \cbr{1, 10, 50}$, with $10$ being the original default.
All other hyperparameters of SDM-WGAN remain the same as in SDM-GAN.
Detail results are presented in Table~\ref{table:jsdipm}.

From the plot of average scores, Figure~\ref{fig:jsd_imp}, we see that the performance of SDM-WGAN is relatively robust to the choice of $\lambda_{\mathrm{GP}}$.
Compared with SDM-GAN, the three variants of SDM-WGAN overall perform worse, and the performances exhibit relatively larger variation across datasets.
Furthermore, the performances of SDM-WGAN are less stable than SDM-GAN, as shown by the relatively larger variance in the results on many tested datasets.
We believe that a thorough guidance to the hyperparameter setups and training schemes for WGAN-GP could potentially improve the performance of SDM-WGAN.
Such guidance is currently missing from the literature.
The investigation onto other instances of IPM, such as the Maximum Mean Discrepancy \citep{kerneltwosampletest2012}, is left as future work.

\begin{table}[ht] 
 \vspace{-6mm}
\caption{
Normalized returns for comparing the default algorithm with variants of approximately matching the Wasserstein-$1$ dual via WGAN-GP.
We vary $\lambda_{\mathrm{GP}} \in \cbr{1, 10, 50}$.
Here ``med" denotes medium, ``rep" for replay, and ``exp" for expert.
} 
\label{table:jsdipm} 
\centering 
\def\arraystretch{1.}
\resizebox{.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
                 Tasks/SDM Variants &           GAN & $\lambda_{\mathrm{GP}} = 1$ & $\lambda_{\mathrm{GP}} = 10$ & $\lambda_{\mathrm{GP}} = 50$ \\
\midrule
              maze2d-umaze &   36.1 {\footnotesize $\pm$ 28.4} &                      26.7 {\footnotesize $\pm$ 42.2} &                       28.4 {\footnotesize $\pm$ 45.2} &                       56.7 {\footnotesize $\pm$ 15.0} \\
             maze2d-med &  115.4 {\footnotesize $\pm$ 34.2} &                       99.8 {\footnotesize $\pm$ 8.0} &                       75.1 {\footnotesize $\pm$ 10.9} &                       96.0 {\footnotesize $\pm$ 10.1} \\
              maze2d-large &  207.7 {\footnotesize $\pm$ 11.7} &                      26.2 {\footnotesize $\pm$ 30.0} &                       44.3 {\footnotesize $\pm$ 63.9} &                         1.5 {\footnotesize $\pm$ 9.5} \\
        halfcheetah-med &    42.5 {\footnotesize $\pm$ 0.5} &                       44.3 {\footnotesize $\pm$ 1.0} &                        45.5 {\footnotesize $\pm$ 0.2} &                        44.4 {\footnotesize $\pm$ 0.6} \\
           walker2d-med &    66.7 {\footnotesize $\pm$ 1.8} &                       9.6 {\footnotesize $\pm$ 12.7} &                       21.6 {\footnotesize $\pm$ 10.7} &                       11.7 {\footnotesize $\pm$ 12.7} \\
             hopper-med &   62.8 {\footnotesize $\pm$ 14.3} &                        9.8 {\footnotesize $\pm$ 9.2} &                         3.5 {\footnotesize $\pm$ 2.9} &                         2.7 {\footnotesize $\pm$ 3.4} \\
 halfcheetah-med-rep &    41.7 {\footnotesize $\pm$ 0.4} &                       49.3 {\footnotesize $\pm$ 0.9} &                        49.3 {\footnotesize $\pm$ 0.6} &                        48.6 {\footnotesize $\pm$ 0.5} \\
    walker2d-med-rep &    20.3 {\footnotesize $\pm$ 4.0} &                      16.2 {\footnotesize $\pm$ 10.7} &                         6.6 {\footnotesize $\pm$ 8.4} &                         8.0 {\footnotesize $\pm$ 6.2} \\
      hopper-med-rep &    30.6 {\footnotesize $\pm$ 2.8} &                       37.2 {\footnotesize $\pm$ 3.1} &                        33.3 {\footnotesize $\pm$ 4.2} &                        28.1 {\footnotesize $\pm$ 3.7} \\
 halfcheetah-med-exp &    89.1 {\footnotesize $\pm$ 6.6} &                       17.1 {\footnotesize $\pm$ 4.7} &                        15.9 {\footnotesize $\pm$ 3.9} &                        22.1 {\footnotesize $\pm$ 6.1} \\
    walker2d-med-exp &    97.9 {\footnotesize $\pm$ 4.9} &                      66.2 {\footnotesize $\pm$ 18.7} &                       56.6 {\footnotesize $\pm$ 23.9} &                        55.3 {\footnotesize $\pm$ 7.8} \\
      hopper-med-exp &   104.5 {\footnotesize $\pm$ 5.4} &                       25.5 {\footnotesize $\pm$ 2.5} &                        25.6 {\footnotesize $\pm$ 5.0} &                        21.3 {\footnotesize $\pm$ 6.3} \\
                 pen-human &    17.8 {\footnotesize $\pm$ 1.7} &                       27.4 {\footnotesize $\pm$ 2.6} &                        24.0 {\footnotesize $\pm$ 7.8} &                        18.7 {\footnotesize $\pm$ 2.9} \\
                pen-cloned &    40.6 {\footnotesize $\pm$ 6.1} &                      46.9 {\footnotesize $\pm$ 18.1} &                       44.0 {\footnotesize $\pm$ 17.4} &                       44.1 {\footnotesize $\pm$ 11.3} \\
                pen-expert &  135.8 {\footnotesize $\pm$ 11.7} &                      63.7 {\footnotesize $\pm$ 26.7} &                       67.1 {\footnotesize $\pm$ 20.7} &                       72.4 {\footnotesize $\pm$ 22.9} \\
               door-expert &    93.5 {\footnotesize $\pm$ 6.7} &                      63.5 {\footnotesize $\pm$ 27.4} &                       50.2 {\footnotesize $\pm$ 36.4} &                       59.1 {\footnotesize $\pm$ 28.8} \\
               \midrule
             Average Score &              75.2 &                                 39.3 &                                  36.9 &                                  36.9 \\
\bottomrule

\end{tabular}
}
% \vspace{-5mm}
\end{table}

==> icml 2022_joint_matching_model_base/Tex/intro.tex <==
\section{Introduction}\label{sec:intro}

% General benefits of offline rl 
Offline reinforcement learning (RL), traditionally known as batch RL, eschews environmental interactions during the policy learning process and focuses on training policy from static dataset collected by one or more data-collecting policies, which we collectively call the behavior policy \citep{treerl2005, batchrl2012, offlinetutorial2020}.
This paradigm extends the applicability of RL from trial-and-error in the simulator \cite{dqn2013,dqn2015,alphago2016,alphazero2017} to applications where environmental interactions can be costly or even dangerous \citep{whentotreat2019,autodrivesurvey2020}, and to domains with abundant accumulated data \citep{offlineabtest2018}.
% Drawbacks of offline RL: distribution-shift 
While classical off-policy RL algorithms \citep{dqn2013,ddpg2016,c512017,qrdqn2017,td32018,sacnew2018} can be directly applied to the offline setting, they often fail to learn purely from a static dataset, especially when the offline dataset exhibits a narrow distribution on the state-action space \citep{bcq2019,bear2019}.
One important cause to such a failure is the mismatch between the stationary state-action distribution of the behavior policy and that of the learned policy, resulting in possibly pathological estimates of the queried action-values during the training process and thus the instability and failure of the policy learning.

To successfully learn a policy from the offline dataset, prior model-free offline RL works try to avoid the action-distribution shift during the training process, so that the overestimated action-values in out-of-distribution (OOD) actions can be mitigated.
Their approaches can be mainly characterized into three categories: 
\textbf{(1)} robustly train the action-value function or provide a conservative estimate of the action-value function whose numerical values distinguish in- and out-of-distribution actions \citep{rem2020,cql2020,addressingextra2021,s4rl2021};
\textbf{(2)} design a tactful behavior-cloning scheme to learn only from ``good" actions in the dataset \citep{crr2020,decisiontrans2021,iql2021};
\textbf{(3)} regularize the current policy to be close to the action choice in the offline dataset during the training process, so that the learned policy mainly takes action within the reach of the action-value function estimate \citep{bcq2019,sibb2019,bear2019,brac2019,offlinerldialog2019,abm2020,oraac2021,fisherbrc2021,uwac2021,td3bc2021}.

Model-based RL (MBRL) can provide a potential enhancement over the model-free RL.
By learning an approximate dynamic model and subsequently using that for policy learning, MBRL can provide a sample-efficient solution to answer the counterfactual question pertaining to action-value estimation in the online setting \citep{mbpo2019,gamembrl2020}, and to provide an augmentation to the static dataset in the offline setting \citep{mopo2020}.
% model based method: still distribution shift so need to constraint the state-action visitation of the learned policy
Directly applying model-based RL methods into the offline setting, however, still faces the challenge of mismatching stationary state-action distribution.
In particular, when the offline dataset only covers a narrow region on the state-action space, the estimated dynamic model may not support far extrapolation \citep{wmopo2021}.
Consequently, poor empirical performance related to the ``model exploitation" issue can appear when directly using the learned model for offline policy learning \citep{asi2012,mbmpo2018,metrpo2018,gamembrl2020,mopo2020}.
As remedies, prior model-based offline RL methods try to avoid state-action pairs far from the offline dataset by uncertainty quantification \citep{mopo2020, morel2020, fan2021contextual,moose2021}, model-based constrained policy optimization \citep{bremen2021,mabe2021}, or model-based conservative action-value function estimation \citep{combo2021}.

% regularize the stationary distribution of the current policy
In this work, we propose to directly regularize the undiscounted stationary state-action distribution of the current policy towards that of the behavior policy during the policy learning process.
The learned policy thus avoids visiting state-action pairs far from the offline dataset, reducing the occurrence of overestimated action-values and stabilizing policy training.
%  train a dynamic model
{
We derive a tractable bound for the distance between the undiscounted stationary distributions.
To implement this bound, we \textbf{(1)} train a dynamic model in a sufficiently rich function class via the maximum likelihood estimation (MLE);
and \textbf{(2)} add a tractable regularizer into the policy optimization objective. This regularizer only requires samples from the offline dataset, the short-horizon model rollouts, the current policy, and the estimated dynamic.}
Further, model-based synthetic rollouts are used to better estimate the stationary state-action distribution of the current policy, which helps the performance of the final policy. 
%the statistical error induced by mismatched stationary distributions and facilitates generalization beyond the static dataset.
% implicit policy
Besides, our framework allows training an implicit policy to better approximate the maximizer of the action-value function estimate, particularly when the latter exhibits multi-modality.
% competitive performance
Without assuming any knowledge about the underlying environment, including the reward function and the termination condition, our method shows competitive performance on a wide range of continuous-control offline-RL datasets from the D4RL benchmark \citep{fu2021d4rl}, validating the effectiveness of our algorithmic designs.
    
    

==> icml 2022_joint_matching_model_base/Tex/main.tex <==
\section{Main Method} \label{sec:main_method}

In this section, we introduce our approach to stabilize the policy training. 
Specifically, except optimizing the policy $\pi$ to maximize the action-value function, we add a distribution regularization into the policy optimization objective, which encourages the closeness between the stationary distribution of the learned policy $\pi$ and that of the behavior $\pi_b$.
Our policy optimization objective is summarized as
\begin{align*}
    J(\pi):= \lambda \E_{s \sim \denv,\, a \sim \pi(\cdot | s)}\sbr{Q_{\vtheta}\br{s, a}} -  D(\dbtrue, \dpitrue),
\end{align*}
where $\lambda$ is the regularization coefficient, $D(\cdot, \cdot)$ is a statistical distance  between two probability distributions, such as the integral probability metric (IPM, \citet{ipm1997}) and the Jensen--Shannon divergence (JSD, \citet{jsd1991}),
$\dbtrue(s,a)$ is the stationary distribution induced by behavior policy $\pi_{b}$ in the true dynamic $P^{*}$, and $\dpitrue(s,a)$ is the stationary distribution induced by the current policy $\pi$ in $P^{*}$.
 
\subsection{A Tractable Bound to the Regularization Term} \label{sec:method_theory}
As discussed in \Secref{sec:background}, the offline dataset $\denv$ is drawn from $\dbtrue$. 
Since the current policy $\pi$ can not interact with the environment during the training process, we can not directly estimate $\dpitrue$ using simulation. 
Hence, we use a learned dynamic model $\widehat P$ to approximate $\dpitrue$. 
Using the triangle inequality for the distance $D$, we have
\begin{align}
    D(\dbtrue, \dpitrue) \leq D(\dbtrue, d_{\pi}^{\widehat P}) + D(d_{\pi}^{\widehat P}, d_{\pi}^{P^*})\,. \label{equ:reg_relax}
\end{align}
Next, we describe how to estimate $D(\dbtrue, d_{\pi}^{\widehat P})$ and how to upper bound $D(d_{\pi}^{\widehat P}, d_{\pi}^{P^*})$ in the RHS of Eq.~\eqref{equ:reg_relax}. % separately. 

{
For a given dynamic model $\widehat P(s^\prime | s,a)$, since we do not know the formula of $d_{\pi}^{\widehat{P}}(s,a)$, a natural way to estimate this distribution is collecting rollouts of $\pi$ on the dynamic $\widehat P$. 
A major drawback of this approach is that it requires drawing many trajectories. 
This can be time-consuming as trajectories are typically long or even infinite, especially when they converge to the stationary distribution slowly. 
Even worse, since $\pi$ changes during the policy-learning process, we have to repeat this expensive rollout process many times.
To estimate $D(\dbtrue, d_{\pi}^{\widehat P})$ in Eq.~\eqref{equ:reg_relax}, we instead derive the following theorem, which avoids sampling full trajectories and only requires sampling a \textit{single} $(s^\prime, a^\prime)$ pair using policy $\pi$ and model $\widehat{P}$ starting from $(s,a)$ drawn from the offline dataset. 
This can significantly save computation and training time.
}

\begin{theorem}\label{prop:ipm1}
If the distance metric $D$ is the IPM w.r.t some function class $\mathcal{G}=\{g: \sS \times \sA \to \mathbb{R}\}$, defined as 
\begin{align*}
    D_{\cG}(\dbtrue, d_{\pi}^{\widehat P}):= \sup_{g\in \mathcal{G}}\left\vert\E_{\dbtrue}\left[g(s,a)\right] - \E_{d_{\pi}^{\widehat P}}\left[g(s,a)\right]\right\vert\,,
\end{align*}
then there exists a $\gG$ s.t. we can rewrite $D_{\cG}(\dbtrue, d_{\pi}^{\widehat P})$ as:
\begin{equation*} 
    \resizebox{.48\textwidth}{!}{%
    $
\begin{aligned}
    &D_{\cG}(\dbtrue, d_{\pi}^{\widehat P})= \mathcal{R}_{\cF}(\dbtrue, \pi,\widehat{P}) \notag \\
    :=&\sup_{f\in \cF} \bigg\vert\E_{(s,a)\sim \dbtrue  }[f(s,a)]-\E_{{s^\prime \sim \widehat P(\cdot | s,a), a^\prime \sim \pi(\cdot | s^\prime)}\atop {(s,a)\sim \dbtrue }}\left[f(s^\prime, a^\prime)\right]\bigg\vert\,, 
\end{aligned}
$%
}
\end{equation*}
where 
\begin{equation*}
    \resizebox{.48\textwidth}{!}{%
$
\begin{aligned}
         \cF:=\Bigg\{f:&~ f(s,a)=\E_{\pi, \widehat{P}}\left[\sum_{t=0}^{\infty}\left(g(s_t,a_t) - \widehat{\eta}^\pi\right)~|~{{a_0=a}\atop{s_0=s}}\right], \, \\
    &\widehat{\eta}^\pi =\lim_{T\to \infty}\E_{\pi, \widehat{P}}\left[\frac{1}{T+1}\sum_{t=0}^{T}g(s_t, a_t)\right], g\in \cG\Bigg\}\,. 
    \end{aligned}
    $%    
}
\end{equation*}
\end{theorem}

We describe the definition of the function class $\gG$ in Appendix~\ref{sec:proof_31}.
In Theorem \ref{prop:ipm1}, the supremum is taken over a new function class $\mathcal{F}$, which captures the \textit{relative value function} following the policy $\pi$ and the transition $\widehat{P}$ when the reward function is the deterministic function $g(s,a)$ \citep{markovdp1994,rlintro2018}. 
{Using this new function class $\gF$ instead of the original $\gG$ enables the aforementioned avoidance of full-trajectory sampling.}
A more detailed discussion on the relation between $f(s,a)$ and $g(s,a)$ can be found in  Appendix \ref{sec:proof_31}.

{
We remark that in practice the relative value function $f$ is approximated by neural networks with regularity, under the same assumptions as approximating the solution of Bellman backup using neural networks.
Because of the expressiveness of neural networks, we assume that $f$ then resides in a richer function class that contains the class $\mathcal{F}$ of differential value functions. 
Since $f$ is maximized over a larger function class than $\gF$, we effectively minimize an upper bound of the original regularization term in Theorem~\ref{prop:ipm1}.
This relaxation avoids explicitly estimating the differential value function for each reward function $g$ encountered in the training process. Such explicit estimation can be time-consuming.
}

Our next step is to bound $D(d_{\pi}^{\widehat P}, d_{\pi}^{P^*})$. 

\begin{theorem}\label{thm:model_error}
Let $P^{*}$ be the true dynamic, $D_\gG$ the IPM with the same $\gG$ as Theorem~\ref{prop:ipm1}, and $\widehat{P}$ the estimated dynamic.
There exist a constant $C \geq 0$ and a function class $\Psi =\{\psi: \sS \times \sA \to \mathbb{R}\}$ such that for any policy $\pi$,
\begin{equation} \label{equ:mb_upper}
    \resizebox{.48\textwidth}{!}{%
$
\begin{aligned}
    D_{\cG}(d_{\pi}^{\widehat P}, d_{\pi}^{P^*}) \leq & C\cdot \E_{(s,a)\sim \dbtrue}\left[\sqrt{\frac{1}{2}\mathrm{KL}\left(P^{*}(s^\prime |s,a) || \widehat{P}(s^\prime | s,a) \right)}\right]   \\
    & \quad +  \mathcal{R}_{\Psi}(\dbtrue, \pi)\,, 
\end{aligned}
    $%    
}
\end{equation}
where 
\begin{equation*}
    \resizebox{.48\textwidth}{!}{%
$
\begin{aligned}
 \mathcal{R}_{\Psi}(\dbtrue, \pi):=\sup_{\psi \in \Psi}\left\vert \E_{(s,a)\sim \dbtrue}[\psi(s,a)] - \E_{s\sim \dbtrue\atop{a\sim \pi(\cdot|s)}}[\psi(s,a)]\right\vert\,.
\end{aligned}
    $%    
}
\end{equation*}
%\yf{TODO: check the description of the assumption}
\end{theorem}
We describe the definition of the function class $\Psi$ in Appendix~\ref{sec:proof_thm_32}. 
Detailed proof of Theorem \ref{thm:model_error} can be found in Appendix \ref{sec:proof_thm_32}. 

\begin{proposition}\label{prop:kl_mle_sec_method}
An upper bound of the first term on the right-hand-side of Eq.~\eqref{equ:mb_upper}
can be minimized via the MLE for $\widehat P$, {\it i.e.}, Eq.~\eqref{eq:model_objective}.
\end{proposition}
Informally, this proposition coincides with the intuition that estimating the environmental dynamic using MLE can be helpful for matching $d_{\pi}^{\widehat P}$ with $d_{\pi}^{P^*}$.
This proposition is restated and proved in Proposition \ref{eq:kl_mle} in Appendix~\ref{sec:proof_thm_32}.

\begin{theorem}\label{col:sum_up}
Combine Theorems \ref{prop:ipm1} and \ref{thm:model_error} and Proposition \ref{prop:kl_mle_sec_method}, and suppose the dynamic model $\widehat P$ is trained by the MLE objective (Eq.~\eqref{eq:model_objective}), then for the same $\gG$ and any policy $\pi$, up to some constants {\it w.r.t.} $\pi$ and $\widehat P$, we have
\begin{equation*}
    \resizebox{.48\textwidth}{!}{%
$
\begin{aligned}
    D_{\cG}(\dbtrue, \dpitrue) \leq \mathcal{R}_{\cF}(\dbtrue, \pi,\widehat{P}) + \mathcal{R}_{\Psi}(\dbtrue, \pi) + \mathcal{E}_{model},
\end{aligned}
    $%    
}
\end{equation*}
where $\mathcal{E}_{model}$ is the error associated with the maximum likelihood training, and is independent of the policy $\pi$.
\end{theorem}
If the function class $\mathcal{P}$ for the estimated dynamic $\widehat P$ is rich enough and we have sufficiently many empirical samples from $\dbtrue$, under the classical statistical regularity condition, we can achieve a small model error $\mathcal{E}_{model}$ by MLE \citep{ferguson1996,casellaberger2001}. 
So we focus on minimizing the first two terms in Theorem~\ref{col:sum_up} as a regularization during the policy improvement step.

\subsection{Practical Implementation} \label{sec:main_method_details}
%\yf{@shentao, can you add some textbf to summary each part for this subsection, the whole subsection are too long for this part and people may loose information, e.g: the first part can add something like model training or model design?}
Based on the analysis in \Secref{sec:method_theory}, we would like to minimize $D_{\cG}(\dbtrue, \dpitrue)$ as a regularization term in the policy optimization step.

\textbf{Model Training.} The first step is to minimize the model error $\mathcal{E}_{model}$ by pre-training the dynamic model under a sufficiently rich function class via MLE.
In this paper, we take on a fully-offline perspective, assuming no prior knowledge about the reward function and the termination condition.
We use neural networks to parameterize the learned transition, reward, and termination.
Following prior model-based offline-RL work \citep{mopo2020,combo2021,mabe2021}, we assume stochastic transition and reward, and use an ensemble of Gaussian probabilistic networks, denoted as $\widehat P(\cdot \given s, a)$ and $\widehat r(s, a)$, to model these distributions.
We use the same model structure, training strategy, and hyperparameters as in \citet{mopo2020}, where the model outputs the mean and log-standard-deviation of the normal distributions of the reward and next state. 
The termination condition is modelled as an ensemble of deterministic sigmoid networks with the same training strategy as $\widehat P$ and $\widehat r$, and outputs the probability of the input satisfying the termination condition.
For computational simplicity, the termination-condition networks share the input and hidden layers with $\widehat P$ and $\widehat r$.
A default cutoff-value of $0.5$ is used to decide termination.
Further details on model training is in Appendix \ref{sec:algo_details_model}.

\paragraph{Model Rollouts.} In practice, we have only a finite static dataset, and we therefore replace sampling from $\dbtrue$ with sampling from its discrete approximation $\denv$.
With the learned model $\widehat P$, we follow prior model-based RL work \citep{mbpo2019, mopo2020} to augment $\denv$ with the replay buffer $\dmodel$ consisting of $h$-horizon rollouts of the current policy $\pi_\vphi$ on the learned model $\widehat P$, by branching from states in the offline dataset $\denv$.
As discussed in \Secref{sec:background}, the augmented dataset is defined as $\gD := f \cdot \denv + (1 - f)\cdot \dmodel$, with $f \in [0,1]$ denotes the percentage of real data.
While theoretically not required in the derivation in \Secref{sec:method_theory}, in our preliminary study we find that adding a significant amount of synthetic rollouts can benefit the performance.
We hypothesize that adding $\dmodel$ can better estimate the stationary state-action distribution of the current policy and hence mitigate the issue of distribution mismatch in offline policy evaluation and optimization.
Besides, $\dmodel$ can also serve as a natural data-augmentation to $\denv$, reducing the sampling error in training the action-value function, as discussed in \citet{combo2021}.
We therefore use $\gD$ in lieu of $\denv$ in the policy evaluation, policy optimization, and regularizer construction.
We follow \citet{combo2021} to use $f=0.5$ for our algorithm and conduct an ablation study on $f$ in \Secref{sec:exp_ablation}.

\textbf{Regularizer Construction.} Though technically possible to use different test functions under different function classes to separately estimate $\mathcal{R}_{\cF}(\dbtrue, \pi,\widehat{P})$ and $\mathcal{R}_{\Psi}(\dbtrue, \pi)$,
for computational simplicity, we use the same test function to directly estimate the sum $\mathcal{R}_{\cF}(\dbtrue, \pi,\widehat{P}) + \mathcal{R}_{\Psi}(\dbtrue, \pi)$, and parametrize the test function using neural network.
%which we follow \citet{repbsde2021} to assume its richness in keep the theoretical bounds (approximately) valid.
We leave the strategy of separate estimation as future work.

A sample-based estimate of $\mathcal{R}_{\cF}(\dbtrue, \pi,\widehat{P}) + \mathcal{R}_{\Psi}(\dbtrue, \pi)$ requires sampling from the data distribution, which we dub as ``true" samples; and sampling from the policy's distribution, dubbed as ``fake" samples.
The ``true" samples $\gB_{\mathrm{true}}$ are formed by sampling from $\denv$.
To form the ``fake" samples $\gB_{\mathrm{fake}}$, we first sample $s \sim \gD$, followed by getting a corresponding action for each $s$ using $a \sim \pi_\vphi(\cdot \given s)$.
Then for each $(s,a)$ pair, we get a sample of the next state $s'$ using the learned model $\widehat P$ as $s' \sim \widehat P(\cdot \given s, a)$, followed by sampling one next action $a'$ for each $s'$ via $a' \sim \pi_\vphi(\cdot \given s')$.
Finally, we construct the ``fake" sample $\gB_{\mathrm{fake}}$ as 
\begin{equation} \label{eq:fake_sample}
\gB_{\mathrm{fake}} :=
\begin{bmatrix}
    (s~, & a~) \\
    (s', & a')
    \end{bmatrix}.
\end{equation}
Here, $(s,a)$ is used to estimate $\E_{s\sim \dbtrue\atop{a\sim \pi(\cdot|s)}}[\psi(s,a)]$, the second term inside the $\abs{\cdot}$ of $\mathcal{R}_{\Psi}(\dbtrue, \pi)$.
The pair $(s',a')$ corresponds to $\E_{{s^\prime \sim \widehat P(\cdot | s,a), a^\prime \sim \pi(\cdot | s^\prime)}\atop {(s,a)\sim \dbtrue }}\left[f(s^\prime, a^\prime)\right]$, the second term inside the absolute-value of $\mathcal{R}_{\cF}(\dbtrue, \pi,\widehat{P})$.

%\yf{@shentao, I feel we should change GAN term to JSD / dual presentation of JSD and perform minimax optimiaztion directly, GAN is not a good word in terms of presentation}
Notice that both the IPM and JSD are well-defined statistical metrics, and matching {\it w.r.t.} one of them effectively matches the other.
Meanwhile, the GAN \citep{gan2014} framework provides a stable training scheme for approximately minimizing JSD, with easy reference to hyperparameter configuration in literature.
We henceforth change the IPM structure in $\mathcal{R}_{\cF}(\dbtrue, \pi,\widehat{P}) + \mathcal{R}_{\Psi}(\dbtrue, \pi)$ to JSD and approximately minimize it via GAN.
This amounts to training a discriminator $D_\vw$ to maximize
\begin{equation}\label{eq:dis_objective}
\textstyle
    \begin{split}
        \frac{1}{\abs{\gB_{\mathrm{true}}}} & \sum_{(s,a)\sim \gB_{\mathrm{true}}}\sbr{\log D_\vw(s,a)} + \\
        & \quad \frac{1}{\abs{\gB_{\mathrm{fake}}}} \sum_{(s,a)\sim \gB_{\mathrm{fake}}} \sbr{\log\br{1-D_\vw(s,a)}},
    \end{split}
\end{equation}
and adding the generator loss $\gL_g(\vphi)$ defined as
\begin{equation} \label{eq:generator_loss}
\textstyle
    \gL_g(\vphi) := \frac{1}{\abs{\gB_{\mathrm{fake}}}} \sum_{(s,a) \in \gB_{\mathrm{fake}}}\sbr{\log\br{1-D_\vw\br{s,a}}}
\end{equation}
as the regularizer into the policy optimization objective.
In the ablation study (\Secref{sec:exp_ablation}), we compare our JSD implementation with minimizing the dual form of Wasserstein-$1$ distance, a special instance of IPM.

\textbf{Critic Training.} Motivated by \citet{bcq2019} and \citet{bear2019}, we use the following critic target:
\begin{equation} \label{eq:q_tilde}
\resizebox{.47\textwidth}{!}{%
$
     \begin{aligned}
         &\widetilde{Q}\br{s, a} \triangleq  r(s,a).\mathrm{clamp}(r_{\mathrm{min}}, r_{\mathrm{max}}) + \\
         & \gamma \E_{a'\sim \pi_{\vphi'}\br{\cdot \given s'}}\sbr{c \min_{j=1,2}Q_{\vtheta'_j}\br{s', a'} + (1-c) \max_{j=1,2}Q_{\vtheta'_j}\br{s', a'}} %
     \end{aligned}
$
}
\end{equation}
with $c=0.75$ as in prior work, $r_{\mathrm{min}} = r_0 - 3 \sigma_r$ and $r_{\mathrm{max}} = r_1 + 3\sigma_r$, where $r_0, r_1, \sigma_r$ respectively denote the minimum, maximum, and standard deviation of the rewards in the offline dataset.
Here we adopt similar %reward-clapping
reward-clipping strategy as \citet{wmopo2021} to mitigate the inaccuracy in the reward model.
Each of the double critic networks is trained to minimize the critic loss over $\br{s, a} \in \gB \sim \gD$, {\it i.e.,} $\forall\, j=1,2$,
\begin{equation}\label{eq:critic_target_main}\textstyle
\resizebox{.425\textwidth}{!}{%
$
    \min_{\vtheta_j}\frac{1}{\abs{\gB}}\sum_{\br{s, a} \in \gB} \mathrm{Huber}\br{ Q_{\vtheta_j}\br{s, a} - \widetilde{Q}(s, a)},
    $
}
\end{equation}
where we replace the usual mean-square-error with the Huber loss $\mathrm{Huber}(\cdot)$ for training stability.

\textbf{Policy Training.} We follow \citet{bear2019} to define the policy optimization objective as
\begin{equation} \label{eq:policy_target}
    \arg\min_{\vphi} -\lambda \cdot\frac{1}{\abs{\gB}} \sum_{s \in \gB, a \sim \pi_\vphi(\cdot \given s)}\sbr{\min_{j=1,2} Q_{\vtheta_j}(s, a)} + \gL_g(\vphi),
\end{equation}
where the regularization coefficient $\lambda$ is constructed similar to \citet{td3bc2021} as $$\lambda = \alpha/Q_{avg},$$ with soft-updated $Q_{avg}$.
We use $\alpha=10$ across all datasets in our main results in \Secref{sec:exp_main}.

% implicit
\textbf{Implicit Policy.} To better approximate the maximizer of the action-value function, instead of the classical deterministic or Gaussian policy, in this paper we use a richer function class, the class of implicit distributions, to define our policy.
Specifically, similar to the generator in the conditional GAN (CGAN, \citet{cgan2014}), our implicit policy uses a deterministic neural network to transform a given noise distribution $p_z(z)$ into the state-conditional action distribution. 
Concretely, given state $s$, 
\begin{equation*} \textstyle 
    a \sim \pi_\vphi(\cdot \given s) = \pi_\vphi(s, z), \text{ with } z \overset{iid}{\sim} p_z(z),
\end{equation*}
where $\pi_\vphi$ is a deterministic network.
\Secref{sec:exp_toy} conducts a toy experiment to show the efficacy of the implicit policy, particularly when fitting distributions with multimodality.

We summarize the main steps of our method Algorithm~\ref{alg:simple}, which is implemented by approximately minimizing JSD via GAN and is dubbed as Stationary Distribution Matching via GAN (SDM-GAN).
Further implementation details are provided in Appendix \ref{sec:algo_details}.

\begin{algorithm}[t]
\caption{SDM-GAN, Main Steps}
\begin{algorithmic}
\label{alg:simple}
\STATE Initialize dynamic model $\widehat P$, policy network $\pi_{\vphi}$, critic network $Q_{\vtheta_1}$ and $Q_{\vtheta_2}$, discriminator network $D_\vw$.
\STATE Train $\widehat P$ using maximum likelihood estimation Eq. \eqref{eq:model_objective}
\FOR{each iteration}
\STATE Rollout $\pi_\vphi$ on $\widehat P$, add the synthetic data into $\dmodel$.
\STATE Sample mini-batch $\gB \sim \gD = f\denv + (1-f) \dmodel$. 
\STATE Get critic target via Eq.~\eqref{eq:q_tilde} and train critics by Eq.~\eqref{eq:critic_target_main}.
\STATE Construct $\gB_{\mathrm{fake}}$ via Eq.~\eqref{eq:fake_sample} and sample $\gB_{\mathrm{true}}\sim \denv$.
\STATE Optimize the discriminator $D_\vw$ using Eq.~\eqref{eq:dis_objective}.
\STATE Calculate generator loss $\gL_g(\vphi)$ using Eq.~\eqref{eq:generator_loss}.
\STATE Optimize policy network $\pi_{\vphi}$ by Eq.~\eqref{eq:policy_target}.
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> icml 2022_joint_matching_model_base/Tex/related.tex <==
\section{Related Work} \label{sec:related_work}
\textbf{Model-free Offline RL.}
This paper is related to a classical yet persistent idea in model-free offline RL, {\it i.e.}, matching the learned policy with the behavior policy so that the learned policy mostly visits state-action pairs similar to the offline dataset.
In literature, several designs have been proposed for this purpose, such as constraining the learned policy towards an estimated behavior policy \citep{bear2019,brac2019,offlinerldialog2019}, a tactful decomposition of the action or the action-value function into a behavior-cloning part and an offset \citep{bcq2019, fisherbrc2021}, modification of the critic-learning objective \citep{algaedice2019,cql2020}.
Our paper adds to the literature by directly matching the undiscounted stationary distribution of the learned policy towards the offline dataset. 
To achieve this, we develop the undiscounted version of the change of variable trick to derive a tractable regularizer for policy optimization, which has been explored only in the discounted case \citep{dualdice2019} in the off-policy evaluation (OPE) literature \citep{jiang16doubly,breakingcurse2018,gendice2020}.
Different from the goal of estimating the performance of some policies using offline data, our goal here is to construct a tractable regularization for policy optimization, which involves a learned transition model trained by MLE.
{\citet{jointmatching2022} recently propose the design of an implicit policy via the CGAN structure, together with several additional enhancing techniques. Our paper improves on this prior work by adopting a model-based approach, which facilitates regularizer construction and mitigates distribution mismatch.}
%OPE literature, and use a learned transition dynamic trained by MLE to 
%implement our method.
%To achieve this, we adopt the DualDICE technique in the OPE literature \citep{dualdice2019} to derive a tractable regularizer for policy optimization, 

\textbf{Model-based Offline RL.}
Similar notion of guiding the policy away from the OOD state-action pairs also persists in model-based offline RL.
In literature, such guidance has been implemented by model-output-based uncertainty quantification \citep{mopo2020, morel2020}, estimation of a conservative action-value function \citep{combo2021}, and regularizing the model-based policy learning with a possibly-adaptive behavior prior \citep{mabe2021,bremen2021}.
Recently, techniques in the OPE literarture has been adopted into policy training and model learning.
\citet{wmopo2021} propose an EM-style iterative training of model and policy, with a density-ratio-based weighted model estimation.
Similar to our work, \citet{repbsde2021} utilize the change of variable technique to train the dynamic, which can potentially improve 
the quality of the representations of the dynamic during the model training. 
%DualDICE trick, but focuses on balancing between the discounted stationary distribution induced by the learned policy and the data distribution, for learning distribution-shift-invariant representation on the state-action space during the model training.
By contrast, our paper uses the model-generated rollouts to implement a tractable bound for directly constraining the undiscounted stationary distribution of the learned policy towards the offline dataset during the policy optimization step.
For algorithmic simplicity, our paper does not apply the technique of uncertainty quantification, learnable behavior prior, advanced design of the dynamic model via the GPT-Transformer \citep{gpt2018,fan2020bayesian,trajectorytransformer2021, zhang2022allsh}, {\it etc.}
These are orthogonal to our method and may further improve the empirical performance.
%\textbf{Off-policy Evaluation (OPE):}

%\textbf{Distribution Matching:}

==> icml 2022_joint_matching_model_base/Tex/theory.tex <==
\subsection{Model-Based Joint Matching}

we denote the true transition model as $ P^{*}$, and the
model we learn as $\widehat{P}.$ 
We denote $d_{\denv}$ as the state-action distribution in the offline dataset $\denv$.
Then for the integral probabiliity metric $D_{\gG}$ and the current policy $\pi$ we have 

\begin{equation*}
    D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\denv}}\leq {D_{\gG}}\br{d_{\pi}^{\widehat{P}},d_{\denv}}+D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}}.
\end{equation*}

The first term we can use similar idea as joint matching to have a
computational regularization, and for the second term, we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & :=\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & :=\sup_{g\in\mathcal{G}}\abs{\mathrm{GAP}(s,a)}
\end{align*}

\begin{align*}
\mathrm{GAP}(s,a) & =(1-\gamma)\mathbb{E}_{s\sim \mu_{0},a\sim\pi}\left[\widehat{Q}^{\pi}(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\\
 & =-\gamma\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot \given s,a),a^{\prime}\sim\pi(\cdot\given s^{\prime})}\left[\widehat{Q}^{\pi}(s^{\prime},a^{\prime})\right]+\gamma\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim\widehat{P}(\cdot\given s, a),a^{\prime}\sim\pi(\cdot\given s ^{\prime})}\left[\widehat{Q}^{\pi}(s^{\prime},a^{\prime})\right]\\
 & =-\gamma\left(\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]\right]\right)\\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[D_{\mathrm{TV}}\left(P^{*}(s^{\prime}\given s,a)\Vert\widehat{P}(s^{\prime}\given s,a)\right)\right]\\
\end{align*}

The problem is that we can not get the sample from $d_{\pi}^{ P^{*}}(s,a)$.
Denote $\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)=D_{\mathrm{TV}}\left(P^{*}(s^{\prime}\given s,a)\Vert\widehat{P}(s^{\prime}\given s,a)\right)$,
then we have 

\begin{align*}
\mathrm{GAP}(s,a) & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathcal{\mathbb{E}}_{(s,a)\sim\denv}\left[\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)\right]+\frac{2\gamma g_{\max}}{1-\gamma}\int\left(\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)\left(d_{\denv}(s,a)-d_{\pi}^{ P^{*}}(s,a)\right)dads\right)\\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim\denv}\sqrt{\frac{1}{2}\mathrm{KL}\br{P^*\Vert\widehat{P}}}+\frac{2\gamma g_{\max}M}{1-\gamma}\int\left(\frac{1}{M}\mathcal{\mathcal{E}}_{\widehat{P}}(s,a)\left(d_{\denv}(s,a)-d_{\pi}^{ P^{*}}(s,a)\right)dads\right)\\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim\denv}\sqrt{\frac{1}{2}\mathrm{KL}\br{P^*\Vert\widehat{P}}}+\frac{2\gamma g_{\max}M}{1-\gamma}\sup_{f\in\mathcal{F}}\left\vert f(s,a)\left(d_{\denv}(s,a)-d_{\pi}^{ P^{*}}(s,a)\right)\right\vert \\
 & \leq\frac{2\gamma g_{\max}}{1-\gamma}\mathbb{E}_{(s,a)\sim\denv}\sqrt{\frac{1}{2}\mathrm{KL}\br{P^*\Vert\widehat{P}}}+\frac{2\gamma g_{\max}M}{1-\gamma} D_{\mathcal{F}}\left(d_{\denv}(s,a),d_{\pi}^{P^{*}}(s,a)\right)
\end{align*}

Similarly using the change of variable trick, the last term becomes 

\begin{align*}
D_{\mathcal{F}}\left(d_{\denv}(s,a), d_{\pi}^{P^*}(s,a)\right) & :=\sup_{f\in\mathcal{F}}\left\vert \mathbb{E}_{(s,a)\sim\denv}\left[f(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{P^*}(s,a)}[f(s,a)]\right\vert \\
 & =\sup_{Q_{f}\in\mathcal{\mathcal{Q}}}\left\vert \mathbb{E}_{(s,a,s^{\prime})\sim\denv,a^{\prime}\sim\pi}\left[Q_{f}(s,a)-\gamma Q_{f}\br{s^{\prime},a^{\prime}}\right]-(1-\gamma)\mathbb{E}_{s\sim \mu_{0},a\sim\pi}\left[Q_{f}(s,a)\right]\right\vert \\
\end{align*}

\subsection{Model-based Joint Matching: Average Case}

we denote the true transition model as $ P^{*}$, and the
model we learnt by maximizing likelihood as $\widehat{P}$.
We denote $d_{\denv}$ as the state-action distribution in the offline dataset $\denv$ and $\pi$ as the current policy.
Then we have 
\begin{equation*}
    D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\denv}}\leq D_{\gG}\br{d_{\pi}^{\widehat{P}},d_{\denv}}+D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}},
\end{equation*}
where the first term is the one we used for optimizing policy. According
to previous change of variable trick, we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{\widehat{P}},d_{\denv}} & :=\text{\ensuremath{\sup_{g\in\mathcal{G}}\abs{\mathbb{E}_{(s,a)\sim\denv}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim\denv,s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[g(s^{\prime},a^{\prime})\right]}\text{}.}}\\
\end{align*}

In practice we can rollout more than 1 step to increase the efficiency
of the model. 

For the second term $D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}}$,
we have 
\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & :=\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
\end{align*}

Define $\widehat{V}^{\pi}(s)$ and $\widehat{Q}^{\pi}(s)$ as the value and
state action value function induced by policy $\pi$ and the learned
transition model $\widehat{P}(s^{\prime}\given s,a)$, then we have
the average Bellman equation

\[
\widehat{\eta}^{\pi}=\lim_{T\to\infty}\mathbb{E}_{\tau\sim p_{\pi}}\left[\frac{1}{T+1}\sum_{t=0}^{\infty}r_{t}\right]=\mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]
\]
\begin{align*}
\widehat{Q}^{\pi}(s,a)-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right] & =g(s,a)-\widehat{\eta}^{\pi}\,,\\
\end{align*}

Then we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & :=\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{\widehat{P}}}\left[g(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)\right]-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert \widehat{\eta}^{\pi}-\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot\given s ,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)-g(s,a)\right]\right\vert \\
 & =\sup_{g\in\mathcal{G}}\left\vert -\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\widehat{Q}^{\pi}(s,a)-g(s,a)+\widehat{\eta}^{\pi}\right]\right\vert \\
 & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert -\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}},s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]+\mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat V^{\pi}(s^{\prime})\right]\right]\right\vert \\
 & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat V^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat V^{\pi}(s^{\prime})\right]\right]\right\vert \\
\end{align*}

If we define $\mathcal{E}\br{s,a;\widehat{V}^{\pi}}:=\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s ,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]$,
and assume $\sup_{\widehat V^\pi \in \gV} \norm{\widehat V^\pi}_{\infty} \leq V_{\mathrm{max}}$, then we know 

\begin{align*}
\mathcal{E}\br{s,a;\widehat{V}^{\pi}} & :=\mathbb{E}_{s^{\prime}\sim P^{*}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}(\cdot\given s,a)}\left[\widehat{V}^{\pi}(s^{\prime})\right]\\
 & =\int\left( P^{*}(\cdot\given s,a)-\widehat{P}(\cdot\given s,a)\right)\widehat{V}^{\pi}\br{s^{\prime}}ds^{\prime}\\
 & \leq V_{\max}\int\left\vert  P^{*}(\cdot\given s,a)-\widehat{P}(\cdot\given s,a)\right\vert ds^{\prime}\\
 & \leq2V_{\max}\,.
\end{align*}

Recall that the total variation distance is a special instance of the integral probability metrics $D_\gG$ when the function class $\gG = \cbr{g: \norm{g}_\infty \leq 1}$ \citep{ipm2009,mmdgangp2018}.

Then we have

\begin{align*}
D_{\gG}\br{d_{\pi}^{ P^{*}},d_{\pi}^{\widehat{P}}} & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\pi}^{ P^{*}}}\left[\mathcal{E}\br{s,a,\widehat{V}^{\pi}}\right]\right\vert \\
 & =\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\denv}}\left[\mathcal{E}\br{s,a,\widehat{V}^{\pi}}\right]+\int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}(s,a)-d_{\denv}(s,a)\right)dads\right\vert \\
 & \leq\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{(s,a)\sim d_{\denv}}\left[\mathcal{E}\br{s,a,\widehat{V}^{\pi}}\right]\right\vert +\sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}(s,a)-d_{\denv}(s,a)\right)dads\right\vert \\
 &\leq \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathcal{E}\br{s,a,\widehat{V}^{\pi}} \right\vert \right]  + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}(s,a)-d_{\denv}(s,a)\right)dads\right\vert \\
 &= V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \mathbb{E}_{s^{\prime}\sim P^{*}}\left[\frac{\widehat{V}^{\pi}(s^{\prime})}{V_{\mathrm{max}}}\right]-\mathbb{E}_{s^{\prime}\sim\widehat{P}}\left[\frac{\widehat{V}^{\pi}(s^{\prime})}{V_{\mathrm{max}}}\right]
 \right\vert \right] + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}-d_{\denv}\right)dads\right\vert \\
 &= V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \mathrm{TV}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)} \right] + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}-d_{\denv}\right)dads\right\vert \\
 &\leq V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sqrt{{1 \over 2} \mathrm{KL}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)}} \right] + \sup_{\widehat{V}^{\pi}\in\mathcal{\mathcal{V}}}\left\vert \int\mathcal{\mathcal{E}}\br{s,a;\widehat{V}^\pi}\left(d_{\pi}^{ P^{*}}-d_{\denv}\right)dads\right\vert
\end{align*}
since $\norm{\frac{\widehat{V}^{\pi}}{V_{\mathrm{max}}}}_\infty \leq 1$, where we use Lemma~\ref{thm:lemma_exchange_sup_exp} to exchange order between $\sup$ and $\E[\cdot]$, and the last bound is from the Pinsker's inequality. 
The first term of the last equation can be minimize via the maximum likelihood estimation on $\widehat P$ since 
\begin{equation*}
    \begin{split}
        & \min_{\widehat P} V_{\mathrm{max}} \mathbb{E}_{(s,a)\sim d_{\denv}} \left[ \sqrt{{1 \over 2} \mathrm{KL}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)}} \right] \\
        \leq&  \min_{\widehat P}  V_{\mathrm{max}}  \sqrt{{1 \over 2} \mathbb{E}_{(s,a)\sim d_{\denv}} \sbr{\mathrm{KL}\br{P^*(\cdot \given s,a) \| \widehat P(\cdot \given s,a)}}}  \\
        =&  \min_{\widehat P} V_{\mathrm{max}} \sqrt{{1\over 2} \mathbb{E}_{(s,a)\sim d_{\denv}}\sbr{\int P^*(s' \given s,a)\br{\log P^*(s' \given s,a) - \log \widehat P(s' \given s,a)} ds'}} \\
        =&  \min_{\widehat P} V_{\mathrm{max}} \sqrt{{1\over 2} \cbr{\mathbb{E}_{(s,a)\sim d_{\denv}}\sbr{\int P^*(s' \given s,a) \log P^*(s' \given s,a) ds'} - \mathbb{E}_{(s,a)\sim d_{\denv}} \sbr{\int P^*(s' \given s,a)\log \widehat P(s' \given s,a) ds'}}}    
        \\ =&  V_{\mathrm{max}} \sqrt{ {1\over 2} \cbr{\mathbb{E}_{(s,a,s')\sim d_{\denv}}\sbr{ \log P^*(s' \given s,a) } + \min_{\widehat P} \cbr{- \mathbb{E}_{(s,a,s')\sim d_{\denv}} \sbr{ \log \widehat P(s' \given s,a)}}}},
    \end{split}
\end{equation*}
where $V_{\mathrm{max}}$ is a constant and the first term inside $\sqrt{\cdot}$ is a constant, and 
\begin{equation*}
    \arg \min_{\widehat P} \cbr{- \mathbb{E}_{(s,a,s')\sim d_{\denv}} \sbr{ \log \widehat P(s' \given s,a)}} = \arg \max_{\widehat P}  \mathbb{E}_{(s,a,s')\sim d_{\denv}} \sbr{ \log \widehat P(s' \given s,a)}
\end{equation*}
which is exactly the model-training objective Equation~\eqref{eq:model_objective}.


==> icml 2022_joint_matching_model_base/math_command.tex <==

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\usepackage{amsmath,amsfonts,bm,amsthm,amssymb,mathrsfs,algorithm,algorithmic}
\usepackage{hyperref,url,booktabs,enumitem,multicol,graphicx,caption,subcaption}

% \newtheorem{theorem}{Theorem}
% \newreptheorem{theorem}{Theorem}
% \newreptheorem{corollary}{Corollary}
% % \newtheorem{lemma}{Lemma}
% \newreptheorem{lemma}{Lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}



\newcommand{\maroon}[1]{\textcolor{maroon}{#1}}
\newcommand{\explain}[2]{\underset{\mathclap{\overset{\uparrow}{#2}}}{#1}}
\newcommand{\explainup}[2]{\overset{\mathclap{\underset{\downarrow}{#2}}}{#1}}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}
\newtheorem{fact}{Fact}
\newtheorem{conjecture}{Conjecture}


% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
%\def\eqref#1{equation~\ref{#1}}
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvi{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vphi{{\bm{\phi}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% caligraphic letters
\def\cM{{\mathcal{M}}}
\def\cS{{\mathcal{S}}}
\def\cR{{\mathcal{R}}}
\def\cA{{\mathcal{A}}}
\def\cP{{\mathcal{P}}}
\def\cG{{\mathcal{G}}}
\def\cF{{\mathcal{F}}}
\def\cD{{\mathcal{D}}}
\def\cD{{\mathcal{E}}}


% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normLzero}{L^0}
\newcommand{\normLone}{L^1}
\newcommand{\normLtwo}{L^2}
\newcommand{\normLp}{L^p}
\newcommand{\normLmax}{L^\infty}

\newcommand{\normlzero}{\ell^0}
\newcommand{\normlone}{\ell^1}
\newcommand{\normltwo}{\ell^2}
\newcommand{\normlp}{\ell^p}
\newcommand{\normlmax}{\ell^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\newcommand{\abs}[1]{\left\vert#1\right\rvert}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\br}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\given}{\,|\,}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\denv}{\gD_{\mathrm{env}}}
\newcommand{\dmodel}{\gD_{\mathrm{model}}}


\newcommand{\dbtrue}{d_{\pi_b}^{P^{*}}}
\newcommand{\dpitrue}{d_{\pi}^{P^{*}}}

\newcommand{\wQ}{{\widehat{Q}}}
\newcommand{\wP}{{\widehat{P}}}
\newcommand{\trueP}{{P^{*}}}



\usepackage{relsize}
\newcommand*{\defeq}{\stackrel{\mathsmaller{\mathsf{def}}}{=}}
